Helion: Enabling Natural Testing of Smart Homes

Prior work has developed numerous systems that test the security and safety of smart homes. For these systems to be applicable in practice, it is necessary to test them with realistic scenarios that represent the use of the smart home, i.e., home automation, in the wild. This demo paper presents the technical details and usage of Helion, a system that uses n-gram language modeling to learn the regularities in user-driven programs, i.e., routines developed for the smart home, and predicts natural scenarios of home automation, i.e., event sequences that reflect realistic home automation usage. We demonstrate the HelionHA platform, developed by integrating Helion with the popular Home Assistant smart home platform. HelionHA allows an end-to-end exploration of Helion's scenarios by executing them as test cases with real and virtual smart home devices.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\tool can generate realistic scenarios which would help a variety of stakeholders in analyzing home automation to fulfill their own security/safety goals. For instance, security and privacy researchers can design and evaluate the security system or policy using realistic smart home scenarios generated by \tool. 


\tool can also be used with smart home platforms, \eg SmartThings, and Home Assistant. In this demo paper, we implemented \tool on Home Assistant Engine, where users can interact with real physical devices. 

==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}


==> macro.tex <==

\usepackage{epsf}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{times}
\usepackage{ifthen}
\usepackage{array}
\usepackage{comment}
\usepackage{url}
\usepackage{cellspace}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{tabularx}
\usepackage{listings}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{wrapfig}
\usepackage{xspace}
\usepackage{enumitem}
\usepackage{footnote}
\usepackage{gensymb}
\usepackage{todonotes}
\usepackage{tabularx}
\usepackage{makecell}
\newboolean{showcomments}

\usepackage[utf8]{inputenc}
\usepackage{tikz}

\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }

\newcommand{\add}[1]{{{\xspace#1}}}
\newcommand{\modify}[1]{{{\xspace#1}}}

\newcommand\KEVIN[1]{{\color{purple} \nb{KEVIN}{#1}}}
\newcommand\revision[1]{{\color{blue}{#1}}}
\newcommand\ADWAIT[1]{{\color{red} \nb{ADWAIT}{#1}}}
\newcommand\SUNIL[1]{{\color{orange} \nb{SUNIL}{#1}}}
\newcommand\DENYS[1]{{\color{blue} \nb{DENYS}{#1}}}
\newcommand\TODO[1]{{\color{red} \nb{TODO}{#1}}}
\newcommand\REF{{\color{blue}[REF]}\xspace}
\newcommand{\tool}{{H$\epsilon$lion}\xspace}
\newcommand{\tools}{{H$\epsilon$lion}'s\xspace}


\newcommand{\gh}{{\sc GH}\xspace}
\newcommand{\ghs}{{\sc GH}'s\xspace}
\newcommand{\ghv}{{GH$_{56}$}\xspace}
\newcommand{\ghvs}{{GH$_{56}$}'s\xspace}
\newcommand{\ghp}{{GH$_{45}$}\xspace}
\newcommand{\ghps}{{GH$_{45}$}'s\xspace}






\newcommand\fix[1]{{\color{blue} \nb{FIX THIS}{#1}}}
\newcommand{\here}{{\color{blue} \nb{***}{CONTINUE HERE}}}
\newcommand{\re}{{\color{red} \textbf{[REFS]}}\xspace}
\newcommand{\xy}{{\color{red} \textbf{XY}}\xspace}

\newcommand{\ie}{\textit{i.e.},\xspace}
\newcommand{\eg}{\textit{e.g.},\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}	

\newcommand{\fnumber}[1]{{$\mathcal{F}_{#1}$}}
\newcommand{\resq}[1]{\textbf{$RQ_{#1}$}}
\newcommand{\finding}[2]{\vspace{0.25em}\noindent{\bf {\em Finding\ {#1}} (\fnumber{{#1}}): {#2}.}}
\newcommand{\secref}[1]{Sec.~\ref{#1}\xspace}
\newcommand{\figref}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\tabref}[1]{Table~\ref{#1}\xspace}
\newcommand{\Phase}{{\sc Phase}\xspace}
\newcommand{\Phases}{{\sc Phase's~}\xspace}
\newcommand{\nest}{{NEST}\xspace}
\newcommand{\hue}{{HUE}\xspace}
\newcommand{\smartthings}{{SmartThings}\xspace}
\newcommand{\ngram}{{n-gram}\xspace}
\newcommand{\ngrams}{{n-grams}\xspace}
\newcommand{\seqstart}{{\sf <s>}\xspace}
\newcommand{\seqend}{{\sf </s>}\xspace}
\newcommand{\sequence}[1]{{\sf \small #1}}
\newcommand{\routine}[2]{{\bf IF} {\sf \small #1} {\bf THEN} {\sf \small #2}}
\newcommand{\sentence}[1]{\seqstart {\em #1}\seqend}
\newcommand{\pnumber[1]}{{$\mathcal{P}_{#1}$}}
\newcommand{\stopreading}{{\color{red} Stop reading here.}}


	\newcommand{\emphquote}[1]{{\emph{`#1'}}\xspace}
	\newcommand{\emphdblquote}[1]{{\emph{``#1''}}\xspace}
	
	\newcommand{\emphbrack}[1]{\emph{[#1]}\xspace}
			
\newcommand{\subj}{\emphbrack{subject}}
	\newcommand{\act}{\emphbrack{action}}
	\newcommand{\obj}{\emphbrack{object}}
	\newcommand{\prep}{\emphbrack{preposition}}
	\newcommand{\objtwo}{\emphbrack{object2}}

	\newcommand*\ciclednum[1]{\raisebox{.5pt}{\textcircled{\raisebox{-.9pt}
	{#1}}}}

\newcommand{\projtodo}[1]{{\color{red}{\bf TODO:}#1}}



\newcounter{taskctr}
\newcommand{\task}[1]{
  \addtocounter{taskctr}{1}
  \vspace{0.5em}\noindent{\bf Task \arabic{taskctr}.} ({\it #1})
}

\newcommand{\myparagraph}[1]{\vspace{0.5em}\noindent{\bf #1}:}

\pagestyle{empty}

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{shadecolor}{rgb}{0.95,0.95,0.95}
\lstset{ %
        language=Java,
        basicstyle=\ttfamily\footnotesize,
        numbers=left,
        numbersep=5pt,
        numberstyle=\tiny,%
        frame=single,
        breaklines=true,
        breakatwhitespace=false,
        breakindent=3pt, %
        captionpos=b,
        commentstyle=\textit,
        identifierstyle=\ttfamily,
        keywordstyle=\ttfamily
}


\setlist[itemize]{leftmargin=*, noitemsep, topsep=1pt}
\setlist[enumerate]{leftmargin=*, noitemsep, topsep=1pt}

\makeatletter
\renewcommand{\paragraph}{%
	\@startsection{paragraph}{4}%
	{\z@}{0.5ex \@plus 0ex \@minus .2ex}{-1em}%
	{\normalfont\normalsize\bfseries}%
}
\makeatother


\makeatletter
\g@addto@macro\normalsize{%
	\setlength\abovedisplayskip{0pt}
	\setlength\belowdisplayskip{0pt}
	\setlength\abovedisplayshortskip{-10pt}
	\setlength\belowdisplayshortskip{0pt}
}
\makeatother


\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=0.5pt] (char) {#1};}}

\DeclareGraphicsExtensions{.pdf,.png}
\graphicspath{{img/}}

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\newcommand{\required}[1]{\section*{\hfil #1\hfil}}                    %
\renewcommand{\refname}{{\hskip 0pt plus 0.1fil minus 0pt} References Cited\hfil}                   %


==> methodology.tex <==
\section{Methodology}
\label{sec:methodology}

==> results.tex <==
\section{Evaluation}
\label{sec:evaluation}

==> usage.tex <==
\section{DEMO WALKTHROUGH}
\label{sec:appendix}
This section presents a walkthrough of the actual demonstration.
\subsection*{Set up \toolHA }
To set up \toolHA, first download the source code from our GitHub repository~\cite{helion-on-home-assistant}. Follow the first three steps (Helion Setup, Home Assistant Setup, Instructions on Modifying Home Assistant Dashboard) from the \inlinesmall{readme.md}. The suggested python version is $3.8$. 

\subsection*{Use \toolHA}
Here is the step by step guidelines to use \toolHA from the dashboard.\\
From the \toolHA dashboard, in the {\em Settings}, user can do the following changes:
\begin{itemize}
    \item {\bf Order}: determines the order of \ngram model of \tool. Users can choose the value of $n$.
    \item {\bf Flavor}: determines the types of scenarios, \ie up flavor generates realistic scenarios and down flavor generates unrealistic scenarios.
    \item {\bf Input events}: takes user's tokens for \tool  as seeds for prediction. 
\end{itemize}

The cards on {\em Input} module show all the input events, i.e., the history/context based on which \tool predicts future events, which the user provides.

Once the user chooses all the configuration settings and clicks the ``Run \tool'' button, the state of each entity in the {\em Output} module will be changed based on the resultant prediction
Moreover, when users click on ``Run Helion'', the event predicted by \tool is shown one at a time instead of populating the dashboard with all the cards. 
Users can click on the ``Next Event'' button to observe more event cards.




